Rethinking the Backward Propagation for Adversarial Transferability

Transfer-based attacks generate adversarial examples on the surrogate model, which can mislead other black-box models without access, making it promising to attack real-world applications. Recently, several works have been proposed to boost adversarial transferability, in which the surrogate model is usually overlooked. In this work, we identify that non-linear layers (e.g., ReLU, max-pooling, etc.) truncate the gradient during backward propagation, making the gradient w.r.t. input image imprecise to the loss function. We hypothesize and empirically validate that such truncation undermines the transferability of adversarial examples. Based on these findings, we propose a novel method called Backward Propagation Attack (BPA) to increase the relevance between the gradient w.r.t. input image and loss function so as to generate adversarial examples with higher transferability. Specifically, BPA adopts a non-monotonic function as the derivative of ReLU and incorporates softmax with temperature to smooth the derivative of max-pooling, thereby mitigating the information loss during the backward propagation of gradients. Empirical results on the ImageNet dataset demonstrate that not only does our method substantially boost the adversarial transferability, but it is also general to existing transfer-based attacks. Code is available at https://github.com/Trustworthy-AI-Group/RPA.

==> 03Methodold.tex <==
\iffalse

\subsection{Preliminaries}

Let $x$ be a benign image, $y$ the corresponding ground-truth label and $f(x;\theta)$ the classifier with parameters $\theta$ that outputs the predicted label. Let $\hat{y}$ be the target label and $J(x,y;\theta)$ denote the loss function of classifier $f$(\eg the cross-entropy loss). The goal of attackers is to find an example $x^{adv}$ within the constraint of $\|x^{adv}-x\|_p <\epsilon$ to mislead the model prediction, $f(x^{adv};\theta)\neq f(x;\theta)=y$ for non-targeted attacks or $f(x^{adv};\theta) = \hat{y}$ for targeted attacks. Here $\|\cdot\|_p$ denotes the $p$-norm distance. For brevity, the following description will focus on non-targeted attacks with $p=\infty$.

Given a classifier $f$ with parameters $\theta$ and a benign sample $x \in \mathcal{X}$ with ground-truth label $y\in \mathcal{Y}$, where $\mathcal{X}$ denotes all the legitimate images and $\mathcal{Y}$ is the output space. The adversarial non-targeted attacks finds an adversary $x^{adv} \in \mathcal{X}$ to mislead the target model:
\begin{equation}
\small
    f(x^{adv};\theta)\neq f(x;\theta)=y \quad\mathrm{\st}\quad \|x^{adv}-x\|_p <\epsilon,
\end{equation}
where $\epsilon$ is the perturbation budget. For targeted attacks the $x^{adv}$ is:
\begin{equation}
\small
    f(x^{adv};\theta) = \hat{y} \neq y \quad\mathrm{\st}\quad \|x^{adv}-x\|_p <\epsilon,
\end{equation}
where $\hat{y}$ is the target label. In the white-box setting, we can regard the attack as an optimization problem that searches an example in the neighborhood of $x$ so as to maximize the loss function $J$ of the target classifier $f$:
\begin{equation}
\small
    x^{adv} = \mathop{\arg\max}\limits_{\|x^{adv}-x\|_p <\epsilon} J(x, y; \theta),
\end{equation}
which is for the setting of non-targeted attack. For the sake of conciseness, we will take non-targeted attacks as the discussion topic below, and the discussion of non-targeted attacks can be inferred easily.

For black-box attacks, a popular and proven idea is to exploit the transferability of adversarial examples: the adversaries crafted for one model can still fool other models. Therefore, black-box attacks can still be regarded as white-box attacks, but the adversarial examples are generated on the surrogate model, not the target model.

The above optimization problem can be solved by gradient descent, which is %the same idea as 
similar to 
the training process of neural networks:
\begin{equation}
\small
    g_x=\frac{\partial J}{\partial x}=\frac{\partial J}{\partial z_{k_a}}\cdot \prod_{i=k_a-1}^0 \ \frac{\partial z_{i+1}}{z_i},
\end{equation}
where $z_i$ is the output of the $i_{th}$ layer of the classifier and $z_0=x$.

Some %scholars 
researchers believe that the generation of adversarial examples and the training of the neural network are very similar problems~\cite{Lin2020Nesterov}, the only difference lies in the direction and object of optimization. Therefore, %scholars have proposed 
many gradient descent schemes have been proposed, including single-step schemes (\eg, FGSM~\cite{goodfellow2015explaining}) and multi-step schemes (\eg., PGD\cite{madry2017towards}). From this perspective, the transferability of adversarial examples is equivalent to the generalization of neural networks. Existing works mainly focus on better optimization algorithms (\eg, MI-FGSM\cite{dong2018boosting}, NI-FGSM\cite{Lin2020Nesterov}) or data enhancement (\eg, VMI-FGSM\cite{wang2021enhancing}, Admix\cite{wang2021admix}) to improve resistance to migration.

%However, existing transfer-based attacks often focus too much on applying the techniques of neural network training to this domain, which is not entirely applicable. 
Recently, some works have begun to focus on the effect of gradient backward propagation on the transferability of adversarial examples. Here we particularly introduce two transfer-based attacks based on gradient modification.



\textbf{SGM}\cite{wu2020skip} argues that skip connections in neural networks are important for the transferability of adversarial examples. By increasing\HK{check} the weight of gradients from skip connections during the backward propagation process, the success rate of transfer-based attacks can be significantly improved:
\begin{equation}
\small
    \frac{\partial z_{i+1}}{\partial z_{i}}=\gamma \frac{\partial f_{i}}{\partial z_{i}}+1,
\end{equation}
where $z_{i}$ and $z_{i+1}$ are the input and output of a residual block respectively (\ie, $z_{i+1}=z_{i}+f_{i}(z_{i})$), and $\gamma \in (0, 1]$ is the decay parameter.

\textbf{LinBP}\cite{guo2020backpropagating} revisits a not very new but definitely noteworthy hypothesis of Goodfellow \etal's~\cite{goodfellow2015explaining} and disclose that the transferability can be enhanced by improving the linearity of DNNs in an appropriate manner, which sets the local derivative of the ReLU layer to all ones, not only pixels greater than zero:
\begin{equation}
\small
    \frac{\partial z_{i+1}}{\partial z_{i}}=\mathbf{1},
\end{equation}
where $z_{i}$ and $z_{i+1}$ are the input and output of a ReLU layer respectively(\ie, $z_{i+1}=\max(z_{i}, 0)$).

\fi

\subsection{Motivation}
\label{motivation}


Both SGM\cite{wu2020skip} and LinBP\cite{guo2020backpropagating} focus on improving the linearity of DNNs. They all maintain the forward propagation, and only modify the backward propagation, ensuring that the neural network's output will not change while improving its linearity. SGM\cite{wu2020skip} pioneered the unmatched forward and backward propagation, and LinBP\cite{guo2020backpropagating} further broke through the limitation of the residual structure, modifying the activation function layers that brought nonlinearity to the neural network. These were truly innovative and insightful concepts. From another perspective, it is worth considering the effects of truncation during forward propagation and the concomitant information loss during backward propagation, which ultimately results in a decrease in inter-layer correlation. For instance, specifically, the ReLU layer will truncate the negative regions to zero during the forward propagation, and the gradients of these regions cannot continue to propagate during the corresponding backward propagation process. As a result, a portion of the gradient information from the subsequent layer is lost, leading to a destroy of inter-layer correlation. Furthermore, this drawback accumulates over propagation due to the nature of the chain rule. 



To simulate the effects of gradient information loss due to truncation, we apply a mask $\mathcal{M}\sim \mathcal{B}(1, p)$ to the input gradients of the first bottleneck and the last bottleneck of ResNet-50~\cite{he2016deep}, respectively. As shown in Figure~\ref{fig:mask_layer1} and Figure~\ref{fig:mask_layer3}, we set each element ... For this issue, we posit that reducing information loss during backward propagation in a judicious manner can lead to the crafting of adversarial examples with enhanced transferability. In CNNs, both ReLU layers and max-pooling layers cause truncation. In order to verify the effect of weakening truncation on adversarial transferability, we respectively modify the local gradients at the truncated positions of the last ReLU layer and the last maximum pooling layer to $l_g$. As shown in Figure~\ref{fig:factor_relu} and Figure~\ref{fig:factor_max}, ...

%For this issue, We have two considerations: first, the modification of the gradient should not be too large, otherwise the excessive mismatch between the function and the derivative and excessive linearity will limit the performance; and second, the nonlinearity of DNNs does not only come from the activation function layers, but also the max-pooling layers.

% TODO!
For the ReLU layer, we hope to modify its derivative to reduce the gradient information loss while maintaining the approximate match between forward and backward propagation. The \textbf{Sigmoid} function, which is a smoothing of the original derivative function, was the first idea we had. But it is positive all the region, leading to lack of diversity. Actually, what we want is a derivative function that will be negative when it is less than a certain value near to zero. Meanwhile, its modification relative to the original derivative function should not be too large. Finally, we found that the derivative function of the \textbf{SiLU} activation function is very suitable for our needs, as shown in Figure~\ref{fig:derivatives}, which will be used as the derivative function we arranged for the ReLU layer:

\begin{equation}
\small
    \frac{\partial z_{i+1}}{\partial z_{i}}=\sigma (z_{i}) \cdot (1+z_{i} \cdot (1-\sigma (z_{i}))),
    \label{relu}
\end{equation}
where $\sigma(\cdot)$ is the Sigmoid function.

For the max-pooling layer, for each operation window $W_I$ of shape $k_h\times k_w$ of the max-pooling layers in DNNs, the forward propagation is:
\begin{equation}
\small
    W_O = \max W_{I_{(i, j)}} \quad \mathrm{\st} \quad i \in [0, k_h), \ j \in [0, k_w).
\end{equation}
And the original backward propagation is:
\begin{equation}
\small
    \frac{\partial W_O}{\partial W_{I_{(i,j)}}} = \left\{ \begin{array}{cc}
        1 & \mathrm{if} \ W_{I_{(i, j)}} = W_O \\
        0 & \mathrm{Otherwise}
    \end{array} \right. \mathrm{\st} \quad i \in [0, k_h), \ j \in [0, k_w).
\end{equation}

We hope to smooth the gradient feature map to reduce the information loss, thereby improving the inter-layer correlations. Additionally, the sum of the local gradient in each window should remain constant at 1. As shown in Figure~\ref{fig:max-pooling}, we choose to use the \textbf{Softmax} function to smooth the gradient calculation formula of the max-pooling layer:
\begin{equation}
\small
    \frac{\partial W_O}{\partial W_{I_{(i,j)}}} = \frac{e^{t \cdot W_{I_{(i, j)}}}}{\sum_{i \in [0, k_h)}\sum_{\ j \in [0, k_w)} e^{t \cdot W_{I_{(i, j)}}}} \quad \mathrm{\st} \quad i \in [0, k_h), \ j \in [0, k_w),
    \label{max-pooling-window}
\end{equation}
where $t\ge 0$ is the temperature coefficient for Softmax function. Then the gradients of sliding windows should be folded together for the input gradient of the max-pooling layer:
\begin{equation}
\small
    \frac{\partial z_{i+1}}{\partial z_{i}}=\mathcal{F}(\mathcal{G}),
    \label{max-pooling}
\end{equation}
where $\mathcal{F}$ is the fold function and $\mathcal{G}$ is the set with gradients calculated by Eq.~\ref{max-pooling-window} of all windows.

\subsection{Backward Propagation Attack}
As mentioned above, we consider selecting several ReLU layers and max-pooling layers in backward propagation, and modify their backward propagation calculation formulas to obtain a better gradient of the input image. Based on these motivations, we propose a novel transfer-based attack, called Backward Propagation Attack(\name), that perform gradient modification on backward propagation in existing attacks.

\input{figures/max-pooling}

\textbf{Perform forward propagation of selected basic method on the surrogate model}. Our method does not conflict with existing attack methods, so it can be easily integrated into these methods. Actuality, no change should be made on these fundamental attack methods during the forward propagation.

\textbf{Conduct backward propagation with gradient modification}. In the process of backward propagation, the local gradients of selected layers are calculated based on Eq.~\ref{relu} or Eq.~\ref{max-pooling}.

\textbf{Use the obtained gradients for later procedures.} The selected basic method may contain momentum operation or the like, and we just follow these completely. The adversarial examples obtained on the surrogate model are then used to attack the target model.

The core innovation of \name lies in the modification of backward propagation, which improves the gradient of the input image, and then a more transferable adversarial example is obtained. The entire algorithm of \name is summarized in Algorithm~\ref{alg}.

\input{algorithm}


==> algorithm.tex <==
\begin{algorithm}[t] 
    \small
    \newcommand\mycommfont[1]{\footnotesize\ttfamily{#1}}
    \SetCommentSty{mycommfont}
    \caption{Improved Backward Propagation}
	\label{alg}
	\KwIn{The cross-entropy loss $\bm{J}$ between the logit and the ground-truth label; All layers $\bm{\mathcal{A}}=\{l_{i}\},(0<=i<k_a)$ of the suggorate model; Outputs $\bm{\mathcal{O}}=\{z_{i}\}, (0<=i<=k_a)$ of every layer; Selected layers $\bm{\mathcal{S}}=\{l_{i}\},(0<=i<k_s)$ for gradient modification; The temperature coefficient $\bm{t}$ for Softmax function.}
        \KwOut{Better gradient $\bm{g}$ of the input image.}
        $g_{k_a} = \frac{\partial J}{\partial z_{k_a}}$; \\
        \For(\Comment{compute gradient by the Chain Rule}){$i=k_a-1 \to 0$}{
            \If{$\mathcal{A}[i] \in \mathcal{S}$}{
                \If{$\mathcal{A}[i]$ is a ReLU layer}{
                    Calculate $g_i=g_{i+1} \cdot \frac{\partial z_{i+1}}{\partial z_i}$ based on Eq.~\ref{relu};
                }
                \Else{
                    Calculate $g_i=g_{i+1} \cdot \frac{\partial z_{i+1}}{\partial z_i}$ based on Eq.~\ref{max-pooling};
                }
            }
            \Else{
                Calculate $g_i=g_{i+1} \cdot \frac{\partial z_{i+1}}{\partial z_i}$ based on standard formula; \algorithmiccomment{no modification}
            }
        }
    \Return $g_0$.\\
\end{algorithm} 

==> figures/backpropagation.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \vspace{-1.1em}
    \includegraphics[width=0.92\linewidth]{figures/backpropagation.pdf}
    \vspace{-0.5em}
    \caption{Illustration of %proposed method. 
    \name. During the backward propagation, several layers (\eg, $SL_i$ and $SL_j$) will be selected for gradient modification.}
    \label{fig:backpropagation}
    \vspace{-2em}
\end{wrapfigure}

==> figures/iterations.tex <==
\begin{figure*}[t]
    \hspace{-1em}
    \begin{subfigure}{.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/iterations_mobilenet.pdf}
    \caption{MobileNet}
    \label{fig:iterations_mobilenet}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/iterations_inception_resnet_v2.pdf}
    \caption{Inception-Resnet-v2}
    \label{fig:iterations_inception_resnet_v2}
    \end{subfigure}%
    \begin{subfigure}{.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/iterations_senet.pdf}
    \caption{SENet}
    \label{fig:iterations_senet}
    \end{subfigure}%
    \vspace{-0.6em}
    \caption{Attack success rate on MobileNet, Inception-Resnet-v2 and SENet with various number of iterations for the back-end MI-FGSM}
    \label{fig:query_succ}
    \vspace{-2.3em}
\end{figure*}

==> figures/max-pooling.tex <==
\begin{wrapfigure}{r}{0.3\textwidth}
    \centering
    \vspace{-2em}
    \includegraphics[width=0.92\linewidth]{figures/max-pooling.pdf}
    \vspace{-0.5em}
    \caption{The max-pooling layer after modification}
    \label{fig:max-pooling}
    \vspace{-2em}
\end{wrapfigure}
